Physics performances for Scalar Electron, Scalar Muon and Scalar Neutrino searches at 3 TeV and 1.4 TeV at CLIC

The determination of scalar lepton and gaugino masses is an important part of the programme of spectroscopic studies of Supersymmetry at a high energy e+e- linear collider. In this article we present results of a study of the processes: e+e- -> eR eR -> e+e- chi0 chi, e+e- -> muR muR -> mu mu- chi0 chi0, e+e- -> eL eL -> e e chi0 chi0 and e+e- -> snu_e snu_e -> e e chi+ chi-in two Supersymmetric benchmark scenarios at 3 TeV and 1.4 TeV at CLIC. We characterize the detector performance, lepton energy resolution and boson mass resolution. We report the accuracy of the production cross section measurements and the eR muR, snu_e, chi+ and chi0 mass determination, estimate the systematic errors affecting the mass measurement and discuss the requirements on the detector time stamping capability and beam polarization. The analysis accounts for the CLIC beam energy spectrum and the dominant beam-induced background. The detector performances are incorporated by full simulation and reconstruction of the events within the framework of the CLIC_ILD_CDR detector concept.

==> fltpoint.tex <==
%%
%% This is file `fltpoint.tex',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% fltpoint.dtx  (with options: `fltmain')
%% 
%% IMPORTANT NOTICE:
%% 
%% For the copyright see the source file.
%% 
%% Any modified versions of this file must be renamed
%% with new filenames distinct from fltpoint.tex.
%% 
%% For distribution of the original source see the terms
%% for copying and modification in the file fltpoint.dtx.
%% 
%% This generated file may be distributed as long as the
%% original source files, as listed above, are part of the
%% same distribution. (The sources need not necessarily be
%% in the same archive or directory.)
\edef\atcatcode{\the\catcode`\@}
\catcode`\@=11
\ifx\documentclass\relax
\long\def\@ifnextchar#1#2#3{%
  \let\reserved@d=#1%
  \def\reserved@a{#2}%
  \def\reserved@b{#3}%
  \futurelet\@let@token\@ifnch}
\def\@ifnch{%
  \ifx\@let@token\@sptoken
    \let\reserved@c\@xifnch
  \else
    \ifx\@let@token\reserved@d
      \let\reserved@c\reserved@a
    \else
      \let\reserved@c\reserved@b
    \fi
  \fi
  \reserved@c}
\def\:{\let\@sptoken= } \:
\def\:{\@xifnch} \expandafter\def\: {\futurelet\@let@token\@ifnch}
\fi
\def\iloop#1\irepeat{\def\ibody{#1}\iiterate}
\def\iiterate{\ibody\let\inext=\iiterate\else\let\inext=\relax\fi
   \inext}
\def\xloop#1\xrepeat{\def\xbody{#1}\xiterate}
\def\xiterate{\xbody\let\xnext\xiterate\else\let\xnext\relax\fi\xnext}
\let\repeat\fi
\let\irepeat\fi
\let\xrepeat\fi
\newcount\fp@loopcount
\newcount\fp@loopcountii
\newcount\fp@result
\newcount\fp@carryover
\newcount\fp@tempcount
\newcount\fp@tempcountii
\def\fp@setparam#1{\xdef\fp@param{#1}}%
\def\ar@set#1#2#3{\expandafter\edef\csname#1@\number#2\endcsname{%
   \number#3}}
\def\ar@get#1#2{\csname#1@\number#2\endcsname}
\def\ar@setsig#1#2{\expandafter\edef\csname#1@sig\endcsname{#2}}
\def\ar@getsig#1{\csname#1@sig\endcsname}
\def\ar@getul#1{\csname#1@ul\endcsname}
\def\ar@getll#1{\csname#1@ll\endcsname}
\def\ar@setul#1#2{\expandafter\edef\csname#1@ul\endcsname{\number#2}}
\def\ar@setll#1#2{\expandafter\edef\csname#1@ll\endcsname{\number#2}}
\def\fp@settomax#1#2#3{%
   \ifnum#2<#3\relax
      #1=#3\relax
   \else
      #1=#2\relax
   \fi
}
\def\fp@settomin#1#2#3{%
   \ifnum#2<#3\relax
      #1=#2\relax
   \else
      #1=#3\relax
   \fi
}
\def\fp@modulo#1#2{%
   \fp@tempcount=#1\relax
   \fp@tempcountii=#1\relax
   \divide\fp@tempcountii#2\relax
   \multiply\fp@tempcountii#2\relax
   \advance\fp@tempcount-\fp@tempcountii
   \edef\fp@param{\number\fp@tempcount}}
\def\fp@regread#1#2{%
   \fp@regread@raw{#1}{#2}%
   \fp@cleanreg{#1}}
\def\fp@regread@raw#1#2{%
   \fp@tempcount=0
   \edef\fp@arrayname{#1}%
   \ar@setsig{#1}{+}%
   \edef\fp@scratch{#2\fp@decimalsign}%
   \expandafter\fp@readchars\fp@scratch\end
   \ifnum\ar@getul{#1}=-1
      \ar@setul{#1}{0}%
      \ar@set{#1}{0}{0}%
   \fi
   \fp@tempcount=0
   \fp@tempcountii=\ar@getul{#1}\relax
   \iloop
   \ifnum\fp@tempcount<\fp@tempcountii
      \edef\fp@scratch{\ar@get{#1}{\fp@tempcountii}}%
      \ar@set{#1}{\fp@tempcountii}{\ar@get{#1}{\fp@tempcount}}%
      \ar@set{#1}{\fp@tempcount}{\fp@scratch}%
      \advance\fp@tempcount by 1
      \advance\fp@tempcountii by -1
   \irepeat
}% end \fp@regread@raw
\def\fp@readchars#1{%
   \ifx#1\end
      \let\inext=\relax
      \ifnum\fp@tempcount<0
         \advance\fp@tempcount by 1
         \ar@setll{\fp@arrayname}{\fp@tempcount}%
      \else
         \ar@setll{\fp@arrayname}{0}%
      \fi
   \else % \ifx#1\end
      \let\inext=\fp@readchars
      \ifx#1+%
      \else
         \ifx#1-%
            \if\ar@getsig{\fp@arrayname}-%
               \ar@setsig{\fp@arrayname}{+}%
            \else
               \ar@setsig{\fp@arrayname}{-}%
            \fi
         \else
            \if\noexpand#1\fp@decimalsign%
               \ifnum\fp@tempcount>-1
                  \advance\fp@tempcount by -1
                  \ar@setul{\fp@arrayname}{\fp@tempcount}%
                  \fp@tempcount=-1
               \fi
            \else
               \ar@set{\fp@arrayname}{\fp@tempcount}{#1}%
               \ifnum\fp@tempcount<0
                  \advance\fp@tempcount by -1
               \else
                  \advance\fp@tempcount by 1
               \fi
            \fi% end \if\noexpand#1\fp@decimalsign
         \fi% end \ifx#1-
      \fi% end \ifx#1+
   \fi% end \ifx#1\end
   \inext
}% end \fp@readchars
\def\fp@regget#1#2{%
   \if\ar@getsig{#1}-%
      \def#2{-}%
   \else
      \def#2{}%
   \fi
   \fp@tempcount=\ar@getul{#1}\relax
   \iloop
      \ifnum\fp@tempcount=-1
         \edef#2{#2\fp@decimalsign}%
      \fi
      \edef#2{#2\ar@get{#1}{\fp@tempcount}}%
   \ifnum\fp@tempcount>\ar@getll{#1}\relax
      \advance\fp@tempcount by -1
   \irepeat
}% end \def\fp@regget
\def\fp@cleanreg#1{%
   \fp@tempcount=\ar@getul{#1}\relax
   \iloop
   \ifnum\fp@tempcount>0
      \ifnum\ar@get{#1}{\fp@tempcount}=0
         \advance\fp@tempcount by -1
         \ar@setul{#1}{\fp@tempcount}%
      \else
         \fp@tempcount=0
      \fi
   \irepeat
   \fp@tempcount=\ar@getll{#1}\relax
   \iloop
   \ifnum\fp@tempcount<0
      \ifnum\ar@get{#1}{\fp@tempcount}=0
         \advance\fp@tempcount by 1
         \ar@setll{#1}{\fp@tempcount}%
      \else
         \fp@tempcount=0
      \fi
   \irepeat
   \ifnum\ar@getll{#1}=\ar@getul{#1}\relax
      \ifnum\ar@get{#1}{0}=0\relax
         \ar@setsig{#1}{+}%
      \fi
   \fi
}% end \fp@regclean
\def\fp@getdigit#1#2{%
   \ifnum#2<\ar@getll{#1}\relax
      \fp@setparam0%
   \else
      \ifnum#2>\ar@getul{#1}\relax
         \fp@setparam0%
      \else
         \fp@setparam{\ar@get{#1}{#2}}%
      \fi
   \fi
}% end \fp@getdigit
\def\fp@shiftright#1#2{%
   \edef\fp@shiftamount{\number#2}%
   \fp@settomax{\fp@tempcount}{\ar@getul{#1}}{-\fp@shiftamount}%
   \fp@settomin{\fp@tempcountii}{\ar@getll{#1}}{-\fp@shiftamount}%
   \def\fp@shiftnum{}%
   \iloop
      \fp@getdigit{#1}{\fp@tempcount}%
      \edef\fp@shiftnum{\fp@shiftnum\fp@param}%
      \ifnum\fp@tempcount=-\fp@shiftamount\relax
         \edef\fp@shiftnum{\fp@shiftnum\fp@decimalsign}%
      \fi
   \ifnum\fp@tempcount>\fp@tempcountii
      \advance\fp@tempcount by -1
   \irepeat
   \fp@regread{#1}{\fp@shiftnum}%
}% end \fp@shiftright
\def\fp@firstnonzero#1{%
   \fp@regcomp{#1}{@0}%
   \if\fp@param=%
      \fp@setparam0%
   \else
      \fp@tempcount=\ar@getul{#1}\relax%
      \fp@tempcountii=\ar@getll{#1}\relax%
      \iloop
         \ifnum\ar@get{#1}{\fp@tempcount}>0
            \fp@setparam{\number\fp@tempcount}%
            \fp@tempcount=\fp@tempcountii
         \fi
      \ifnum\fp@tempcount>\fp@tempcountii
         \advance\fp@tempcount by -1
      \irepeat
   \fi
}% end \fp@firstnonzero
\def\fp@regcomp#1#2{%
   {%
      \if\ar@getsig{#1}-%
         \if\ar@getsig{#2}-%
            \fp@regcomp@main{#1}{#2}<>%
         \else
            \fp@setparam{<}%
         \fi
      \else
         \if\ar@getsig{#2}-%
            \fp@setparam{>}%
         \else
            \fp@regcomp@main{#1}{#2}><%
         \fi
      \fi
   }%
}
\def\fp@regcomp@main#1#2#3#4{%
   \fp@settomax{\fp@loopcount}{\ar@getul{#1}}{\ar@getul{#2}}%
   \fp@settomin{\fp@loopcountii}{\ar@getll{#1}}{\ar@getll{#2}}%
   \loop
      \fp@getdigit{#1}{\fp@loopcount}%
      \fp@tempcount=\fp@param\relax
      \fp@getdigit{#2}{\fp@loopcount}%
      \fp@tempcountii=\fp@param\relax
      \ifnum\fp@tempcount<\fp@tempcountii
         \fp@setparam{#4}%
         \fp@loopcount=\fp@loopcountii
      \else
         \ifnum\fp@tempcount>\fp@tempcountii
            \fp@setparam{#3}%
            \fp@loopcount=\fp@loopcountii
         \else
            \ifnum\fp@loopcount=\fp@loopcountii
               \fp@setparam{=}%
            \fi
         \fi
      \fi
   \ifnum\fp@loopcount>\fp@loopcountii
      \advance\fp@loopcount by -1
   \repeat
}% end \fp@regcomp@main
\def\fp@regabs#1{%
   \ar@setsig{#1}{+}%
}
\def\fp@regneg#1{%
   \if\ar@getsig{#1}-%
      \ar@setsig{#1}{+}%
   \else
      \fp@regcomp{#1}{@0}%
      \if\fp@param=%
      \else
         \ar@setsig{#1}{-}%
      \fi
   \fi
}
\def\fp@reground#1#2{%
   \ifnum#2>\ar@getll{#1}\relax
      {%
         \fp@tempcount=#2\relax
         \advance\fp@tempcount by -1
         \fp@getdigit{#1}{\fp@tempcount}%
         \ifnum\fp@param>4
            \fp@regcopy{fp@temp}{@1}%
            \fp@shiftright{fp@temp}{#2}%
            \fp@regcomp{#1}{@0}%
            \if\fp@param<%
               \fp@regneg{fp@temp}%
            \fi
            \fp@regadd{#1}{fp@temp}%
         \fi
         \ifnum#2>0
            \fp@loopcount=#2\relax
            \iloop
               \ifnum\fp@loopcount>0
                  \advance\fp@loopcount by -1
                  \ar@set{#1}{\fp@loopcount}{0}%
            \irepeat
            \ar@setll{#1}{0}%
         \else
            \ar@setll{#1}{#2}%
         \fi
         \fp@regget{#1}{\fp@scratch}%
         \fp@setparam\fp@scratch
      }%
      \fp@regread{#1}{\fp@param}%
   \fi
} % end \fp@reground
\def\fp@regcopy#1#2{%
   \fp@regget{#2}{\fp@scratch}%
   \fp@regread{#1}{\fp@scratch}%
}
\def\fp@regadd#1#2{%
   {%
      \if\ar@getsig{#1}\ar@getsig{#2}%
         \fp@settomin{\fp@loopcount}{\ar@getll{#1}}{\ar@getll{#2}}%
         \edef\fp@add@start{\number\fp@loopcount}%
         \fp@settomax{\fp@tempcount}{\ar@getul{#1}}{\ar@getul{#2}}%
         \edef\fp@add@finish{\number\fp@tempcount}%
         \fp@carryover=0
         \loop
            \fp@getdigit{#1}{\fp@loopcount}%
            \fp@result=\fp@param\relax
            \fp@getdigit{#2}{\fp@loopcount}%
            \advance\fp@result by \fp@param\relax
            \advance\fp@result by \fp@carryover
            \ifnum\fp@result>9
               \fp@carryover=1
               \advance\fp@result by -10
            \else
               \fp@carryover=0
            \fi
            \ar@set{#1}{\fp@loopcount}{\fp@result}%
         \ifnum\fp@loopcount<\fp@add@finish\relax
            \advance\fp@loopcount by 1
         \repeat
         \ifnum\fp@carryover>0
            \advance\fp@loopcount by 1
            \ar@set{#1}{\fp@loopcount}{\fp@carryover}%
         \fi
         \ar@setll{#1}{\fp@add@start}%
         \ar@setul{#1}{\fp@loopcount}%
         \fp@regget{#1}{\fp@scratch}%
         \fp@setparam\fp@scratch
      \else % \if sign
         \fp@regcopy{fp@tempi}{#1}%
         \fp@regcopy{fp@tempii}{#2}%
         \fp@regabs{fp@tempi}%
         \fp@regabs{fp@tempii}%
         \fp@regcomp{fp@tempi}{fp@tempii}%
         \if\fp@param>%
            \fp@regadd@sub{#1}{fp@tempi}{fp@tempii}%
         \else
            \fp@regadd@sub{#2}{fp@tempii}{fp@tempi}%
         \fi
      \fi % end \if sign
   }%
   \fp@regread{#1}{\fp@param}%
}% end \fp@regadd
\def\fp@regadd@sub#1#2#3{%
   \fp@regsub@restricted{#2}{#3}%
   \fp@regcomp{#1}{@0}%
   \if\fp@param<%
      \fp@regneg{#2}%
   \fi
   \fp@regget{#2}{\fp@scratch}%
   \fp@setparam\fp@scratch
}% end \fp@regadd@sub
\def\fp@regsub@restricted#1#2{%
   {%
      \fp@settomin{\fp@loopcount}{\ar@getll{#1}}{\ar@getll{#2}}%
      \edef\fp@lowermin{\number\fp@loopcount}%
      \fp@settomax{\fp@tempcount}{\ar@getul{#1}}{\ar@getul{#2}}%
      \edef\fp@uppermin{\number\fp@tempcount}%
      \fp@carryover=0
      \loop
         \fp@getdigit{#1}{\fp@loopcount}%
         \fp@result=\fp@param\relax
         \fp@getdigit{#2}{\fp@loopcount}%
         \advance\fp@result by -\fp@param\relax
         \advance\fp@result by \fp@carryover
         \ifnum\fp@result<0
            \fp@carryover=-1
            \advance\fp@result by 10
         \else
            \fp@carryover=0
         \fi
         \ar@set{#1}{\fp@loopcount}{\fp@result}%
      \ifnum\fp@loopcount<\fp@uppermin\relax
         \advance\fp@loopcount by 1
      \repeat
      \ifnum\fp@carryover=-1
         \advance\fp@loopcount by 1
         \ar@set{#1}{\fp@loopcount}{-1}%
      \fi
      \ar@setll{#1}{\fp@lowermin}%
      \ar@setul{#1}{\fp@loopcount}%
   \fp@regget{#1}{\fp@scratch}%
   \fp@setparam\fp@scratch
   }%
   \fp@regread{#1}{\fp@param}%
}% end \fp@regsub@restricted
\def\fp@regsub#1#2{%
   {%
      \fp@regneg{#2}%
      \fp@regadd{#1}{#2}%
      \fp@regget{#1}{\fp@scratch}%
      \fp@setparam\fp@scratch
   }%
   \fp@regread{#1}{\fp@param}%
}
\def\fp@regmul#1#2{%
   {%
      \fp@regcopy{fp@temp1}{@0}%
      \fp@loopcountii=\ar@getll{#2}\relax
      \xloop
         \fp@loopcount=\ar@getll{#1}\relax
         \fp@carryover=0
         \def\fp@newnum{}%
         \loop
            \fp@result=\ar@get{#2}{\fp@loopcountii}\relax
            \multiply\fp@result by \ar@get{#1}{\fp@loopcount}\relax
            \advance\fp@result by \fp@carryover
            \ifnum\fp@result>9
               \fp@carryover=\fp@result
               \divide\fp@carryover by 10
               \fp@tempcount=\fp@carryover
               \multiply\fp@tempcount by 10
               \advance\fp@result by -\fp@tempcount
            \else
               \fp@carryover=0
            \fi
            \edef\fp@newnum{\number\fp@result\fp@newnum}%
         \ifnum\fp@loopcount<\ar@getul{#1}\relax
            \advance\fp@loopcount by 1
         \repeat
         \edef\fp@newnum{\number\fp@carryover\fp@newnum}%
         \fp@regread{fp@temp2}{\fp@newnum}%
         \fp@tempcount=\fp@loopcountii
         \advance\fp@tempcount by -\number\ar@getll{#2}\relax
         \fp@shiftright{fp@temp2}{\fp@tempcount}%
         \fp@regadd{fp@temp1}{fp@temp2}%
      \ifnum\fp@loopcountii<\ar@getul{#2}\relax
         \advance\fp@loopcountii by 1
      \xrepeat
      \fp@tempcount=\ar@getll{#1}\relax
      \advance\fp@tempcount by \ar@getll{#2}\relax
      \fp@shiftright{fp@temp1}{\fp@tempcount}%
      \if\ar@getsig{#1}\ar@getsig{#2}%
      \else
         \fp@regneg{fp@temp1}%
      \fi
   \fp@regget{fp@temp1}{\fp@scratch}%
   \fp@setparam\fp@scratch
   }%
   \fp@regread{#1}{\fp@param}%
} % end \fp@regmul
\def\fp@regdiv#1#2{%
   {%
      \fp@regcopy{fp@temp1}{#1}%
      \fp@regcopy{fp@temp2}{#2}%
      \fp@regabs{fp@temp1}%
      \fp@regabs{fp@temp2}%
      \fp@firstnonzero{fp@temp1}%
      \fp@loopcountii=\fp@param\relax
      \fp@firstnonzero{fp@temp2}%
      \advance\fp@loopcountii by -\fp@param\relax
      \fp@shiftright{fp@temp2}{\fp@loopcountii}%
      \def\fp@divnum{}%
      \ifnum\fp@loopcountii<0
         \fp@tempcount=\fp@loopcountii
         \loop
         \ifnum\fp@tempcount<-1
            \edef\fp@divnum{0\fp@divnum}%
            \advance\fp@tempcount by 1
         \repeat
         \edef\fp@divnum{\fp@decimalsign\fp@divnum}%
      \fi
      \xloop
      \fp@tempcount=\fp@loopcountii
      \advance\fp@tempcount by 1
      \ifnum\fp@tempcount>-\fp@accuracy\relax
         \fp@loopcount=0
         \loop
            \fp@regcomp{fp@temp2}{fp@temp1}%
            \if\fp@param=%
               \def\fp@accuracy{0}%
               \gdef\fp@param{<}%
            \fi
         \if\fp@param<%
            \fp@regsub@restricted{fp@temp1}{fp@temp2}%
            \advance\fp@loopcount by 1
         \repeat
         \ifnum\fp@loopcountii=-1
            \edef\fp@divnum{\fp@divnum\fp@decimalsign}%
         \fi
         \edef\fp@divnum{\fp@divnum\number\fp@loopcount}%
         \fp@shiftright{fp@temp2}{-1}%
         \advance\fp@loopcountii by -1
      \xrepeat
      \if\ar@getsig{#1}\ar@getsig{#2}%
         \fp@regread{fp@temp1}{\fp@divnum}%
      \else
         \fp@regread{fp@temp1}{-\fp@divnum}%
      \fi
      \fp@regget{fp@temp1}{\fp@scratch}%
      \fp@setparam\fp@scratch
   }%
   \fp@regread{#1}{\fp@param}%
}
\def\fp@call@bin#1#2#3#4{%
   {%
      \fp@regread{fp@user1}{#2}%
      \fp@regread{fp@user2}{#3}%
      \csname fp@reg#4\endcsname{fp@user1}{fp@user2}%
      \fp@regget{fp@user1}{\fp@scratch}%
      \fp@setparam\fp@scratch
   }%
   \edef#1{\fp@param}%
}
\def\fpAdd#1#2#3{\fp@call@bin{#1}{#2}{#3}{add}}
\def\fpSub#1#2#3{\fp@call@bin{#1}{#2}{#3}{sub}}
\def\fpMul#1#2#3{\fp@call@bin{#1}{#2}{#3}{mul}}
\def\fpDiv#1#2#3{\fp@call@bin{#1}{#2}{#3}{div}}
\def\fp@call@un#1#2#3{%
   {%
      \fp@regread{fp@user1}{#2}%
      \csname fp@reg#3\endcsname{fp@user1}%
      \fp@regget{fp@user1}{\fp@scratch}%
      \fp@setparam\fp@scratch
   }%
   \edef#1{\fp@param}%
}
\def\fpAbs#1#2{\fp@call@un{#1}{#2}{abs}}
\def\fpNeg#1#2{\fp@call@un{#1}{#2}{neg}}
\def\fpRound#1#2#3{%
   {%
      \fpRegSet{fp@user1}{#2}%
      \fpRegRound{fp@user1}{#3}%
      \fpRegGet{fp@user1}{\fp@scratch}%
      \fp@setparam\fp@scratch
   }%
   \edef#1{\fp@param}%
}
\def\fpRegSet#1#2{\fp@regread{#1}{#2}}
\def\fpRegGet#1#2{\fp@regget{#1}{#2}}
\def\fpRegAdd#1#2{\fp@regadd{#1}{#2}}
\def\fpRegSub#1#2{\fp@regsub{#1}{#2}}
\def\fpRegMul#1#2{\fp@regmul{#1}{#2}}
\def\fpRegDiv#1#2{\fp@regdiv{#1}{#2}}
\def\fpRegAbs#1{\fp@regabs{#1}}
\def\fpRegNeg#1{\fp@regneg{#1}}
\def\fpRegCopy#1#2{\fp@regcopy{#1}{#2}}
\def\fpRegRound#1#2{\fp@reground{#1}{#2}}
\def\fpAccuracy#1{\edef\fp@accuracy{#1}}
\fpAccuracy{5}
\def\fpDecimalSign#1{\edef\fp@decimalsign{#1}}
\fpDecimalSign{,}
\def\fpThousandSep#1{\edef\fp@thousandsep{#1}}
\fpThousandSep{}
\fp@regread{@0}{0}
\fp@regread{@1}{1}
\catcode`\@=\atcatcode\relax
\endinput
%%
%% End of file `fltpoint.tex'.

